Leveraging Distributional Bias for Reactive Collision Avoidance under Uncertainty: A Kernel Embedding Approach

Many commodity sensors that measure the robot and dynamic obstacle's state have non-Gaussian noise characteristics. Yet, many current approaches treat the underlying-uncertainty in motion and perception as Gaussian, primarily to ensure computational tractability. On the other hand, existing planners working with non-Gaussian uncertainty do not shed light on leveraging distributional characteristics of motion and perception noise, such as bias for efficient collision avoidance. This paper fills this gap by interpreting reactive collision avoidance as a distribution matching problem between the collision constraint violations and Dirac Delta distribution. To ensure fast reactivity in the planner, we embed each distribution in Reproducing Kernel Hilbert Space and reformulate the distribution matching as minimizing the Maximum Mean Discrepancy (MMD) between the two distributions. We show that evaluating the MMD for a given control input boils down to just matrix-matrix products. We leverage this insight to develop a simple control sampling approach for reactive collision avoidance with dynamic and uncertain obstacles. We advance the state-of-the-art in two respects. First, we conduct an extensive empirical study to show that our planner can infer distributional bias from sample-level information. Consequently, it uses this insight to guide the robot to good homotopy. We also highlight how a Gaussian approximation of the underlying uncertainty can lose the bias estimate and guide the robot to unfavorable states with a high collision probability. Second, we show tangible comparative advantages of the proposed distribution matching approach for collision avoidance with previous non-parametric and Gaussian approximated methods of reactive collision avoidance.

==> chapters/results_latest.tex <==


\section{Results and Discussion}
\label{Results}
% \Madhav{Use this text as I feel the simulations section needs a complete overhaul}
% \begin{figure}

%     \begin{subfigure}{.49\textwidth}
%         \includegraphics[width=.99\textwidth]{images/current_dist.png}
%         \caption{\small Multi-model Distribution }

%         \includegraphics[width=.99\textwidth]{images/biased.png}
%         \caption{\small Biased Distribution}
%     \end{subfigure}  
%     \caption{\small Distributions used for noise characterization}
%     \label{noise}
% \end{figure}


\noindent \textbf{Implementation Details:} All the simulations were carried out on a desktop in python. The CPU and GPU used were AMD Ryzen 5 3500 and NVIDIA 1660 Super respectively. Ten thousand samples for the agent and the obstacles each were used to model the uncertainty in the state and velocity, where the samples were drawn from multi-model distributions. In addition to that, we used 625 control samples in linear and angular velocity for the agent. In all the plots, the blue circle represents the agent's actual position, the yellow circle represents the obstacle' position, and the lighter shade circles surrounding both the agent and the obstacle represents uncertainty in position. We are calling our approach as 'MMD Dirac Delta' while comparing with other methods. The value of the hyperparameter $/gamma$ used is $0.1$. The method of modelling noise as a Gaussian approximation of the actual noise will referred as 'MMD Gaussian'. One of the other methods whoch is also a distribution matching method which uses KL divergence between two distributions will be called KLD\cite{mmd}. The method that models uncertainty based on chance constraints will be called 'PVO'\cite{pvo}. The larger light blue circle surrounding the agent depicts the sensing area for obstacles. Further qualitative results and the code can be found at \href{https://github.com/anishgupta31296/MMD-with-Dirac-Delta-Distribution}{https://github.com/anishgupta31296/MMD-with-Dirac-Delta-Distribution}.


\subsection{Qualitative Results}
\subsubsection{Validation of Distribution Matching}
Figure \ref{dist_match} shows various stages of collision avoidance for single obstacle. The desired distribution shifts starts coinciding with the dirac-delta distribution as we are avoiding increasing number of samples. The distribution is completely matched at the final stage of collision avoidance.
\begin{figure*}
    \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/g=0.1initialdist.png}\hfill
            \caption{\small \rightskip=0.5cm The collision constraint violation distribution just as the beginning of Collision Avoidance. All samples to the right of 0 indicates the entire distribution of the robot is in collision}
    \end{subfigure}
    \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/g=0.1interdist.png}\hfill
            \caption{\small \rightskip=0.5cm As avoidance maneuver begins, some part of the collision violation distribution coincides with the Dirac Delta Distribution}
    \end{subfigure}
    \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/g=0.1dist.png}\hfill
            \caption{\small \rightskip=0.5cm Towards the end of the collision avoidance maneuver, the distribution of collision violations becomes close to a Dirac function}
    \end{subfigure}
    \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/g=0.1initialdistmatch.png}\hfill
    \end{subfigure}
    \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/g=0.1interdistmatch.png}\hfill
    \end{subfigure}
    \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/dist-0028.png}\hfill
    \end{subfigure}
    \caption{\small Distribution matching taking place for single obstacle case \normalsize}
    \label{dist_match}
\end{figure*}


\subsubsection{Homotopy Selection}
The consequence on eventual outcomes in terms of successful collision avoidance or the lack of it is shown in Figures\ref{side selection}a-f in the single obstacle case. Figure\ref{side selection}a shows successful avoidance with zero overlap in the state uncertainties and correspondingly in figure Figure\ref{side selection}b, the entire distribution of collision violation is shifted to the left indicative of successful avoidance. It is to be noted that the distribution of collision violations is shown without the max operator so that the part of the distribution that is left of zero is not floored at zero thereby admitting negative values. Whereas in figure Figure\ref{side selection}d results in collision as a consequence of approximating the distribution as a Gaussian thereby underestimating the larger spread on the incorrect side. The corresponding distribution of collision violations is shown in figure Figure\ref{side selection}e wherein a fair amount of the distribution continues to lie on the right side indicative of non zero finite probability of collisions, one such instance of it is shown in figure Figure\ref{side selection}c.

\begin{figure*}
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/1 obs biased/Right/0070.png}
        \caption{\small Correct Side chosen}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/1 obs biased/correct side.png}
        \caption{\small Correct Side Distribution}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/1 obs biased/1.png}
        \caption{\small Correct Side Distribution for Gaussian Approximation of noise}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/1 obs biased/Right/0053.png}
        \caption{\small Incorrect Side chosen}
    \end{subfigure}    
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/1 obs biased/wrong side.png}
        \caption{\small Incorrect Side Distribution}
    \end{subfigure} 
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/1 obs biased/2.png}
        \caption{\small Incorrect Side Distribution for Gaussian Approximation of noise}
    \end{subfigure}
    \caption{\small Effect of selecting correct side on collision cone distribution \normalsize}
     \label{side selection}

\end{figure*}
\begin{figure*}
   \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/3 obs/0006.png}\hfill
    \end{subfigure}
    \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/3 obs/0049.png}\hfill
    \end{subfigure}
    \begin{subfigure} {.33\textwidth}
            \includegraphics[width=.9\textwidth]{images/3 obs/0088.png}\hfill
    \end{subfigure}
    \begin{subfigure} {.99\textwidth}
            \begin{center}
             \includegraphics[width=.9\textwidth]{images/3 obs/3 obs dist correct side.png}\hfill
            \end{center}
     \label{3obsMMDDiracDelta}
    \end{subfigure}
     \caption{\small Collision avoidance using MMD Non Gaussian for 3 obstacle case \normalsize}
     \label{3 obs}
\end{figure*}

\subsubsection{Other Qualitative Results}
Figures \ref{3 obs} and \ref{4 obs}
showcase the robustness of our algorithm in cases of multiple obstacles. By showcasing the ability of the algorithm where many samples of the ego robot is able to avoid many samples of the obstacles and for many such obstacles we verify its efficiency. 

\begin{figure*}
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/4 obs/0006.png}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/4 obs/0073.png}
    \end{subfigure}    
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.9\textwidth]{images/4 obs/0142.png}
    \end{subfigure}  
     \caption{\small Collision avoidance using MMD Non Gaussian for 4 obstacle case \normalsize}
     \label{4 obs}
\end{figure*}

\subsection{Ablation Studies}
\subsubsection{Empirical Analysis}
\subsubsection{Empirical Analysis}



